Orbia: Do Generated Videos Form a Consistent 3D World?

Video generators serve as interactive worlds for exploration and simulation, yet realistic and visually appealing frames do not necessarily depict a consistent 3D world. Existing benchmarks assess selected geometric properties or use vision-language models to judge memory and consistency, leaving systematic 3D evaluation underexplored. We introduce Orbia, the first benchmark dedicated to a systematic and comprehensive evaluation of 3D consistency in interactive world models. Through controlled exploration and revisit, we organize the evaluation into three dimensions: input preservation, generated-content persistence, and 3D self-consistency. For input preservation, registered RGB-D references and annotated anchors support appearance, geometry, and spatial stability measurements. For generated-content persistence, we compare revisits to regions absent from the input image with their first generated observations to test whether models preserve what they create. For 3D self-consistency, cross-view depth and feature correspondence, regional scale agreement, and held-out Gaussian rendering test whether generated views describe the same 3D scene. Minute-long exploration and revisits further test long-term consistency. Our construction and annotation pipeline brings together public datasets, self-captured scenes, and simulation, yielding 720 instances across indoor and outdoor environments and six exploration-and-revisit protocols. Evaluation spans 27 text-, action-, and camera-conditioned models through native-interface adapters. Our Orbia benchmark provides a systematic basis for diagnosing 3D inconsistency and developing more persistent video world models.

==> paper-macros.tex <==
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta,positioning,calc}
\DeclareFontShape{T1}{optimistic}{b}{sc}{<-> s * [0.88] \reportfontpath/optimistic}{}
\DeclareFontShape{T1}{optimistic}{b}{it}{<->ssub * cmss/bx/sl}{}
\DeclareMathSizes{7.5}{7}{5}{5} %
\urlstyle{rm}
\definecolor{coherence}{HTML}{2866A8}
\definecolor{evidence}{HTML}{B58A38}
\definecolor{persistence}{HTML}{388F80}
\definecolor{muted}{HTML}{657481}
\DeclareRobustCommand{\orbia}{%
  \texorpdfstring{\orbiaGradientText{\textbf{\textsc{Orbia}}}}{Orbia}}

\pdfmapline{+ComicNeue-Bold-tlf-ot1 ComicNeue-Bold "AutoEnc_trnund3iw5ps7cxtmzq5pkl5me ReEncodeFont" <[fonts/comicneue/a_trnund.enc <fonts/comicneue/ComicNeue-Bold.pfb}
\DeclareFontFamily{OT1}{orbiacomic}{}
\DeclareFontShape{OT1}{orbiacomic}{b}{n}{<-> fonts/comicneue/ComicNeue-Bold-tlf-ot1}{}
\newcommand{\referencefont}{\fontencoding{OT1}\fontfamily{orbiacomic}\fontseries{b}\fontshape{n}\selectfont}

\newlength{\dimensioncardgap}
\setlength{\dimensioncardgap}{8pt}
\newcommand{\dimensioncard}[3]{%
  \par\addvspace{\dimensioncardgap}\noindent
  \begingroup
  \setlength{\fboxsep}{6pt}%
  \colorbox{#1!6}{%
    \begin{minipage}{\dimexpr\linewidth-2\fboxsep\relax}
      \textcolor{#1}{\textbf{#2}}\par
      #3
    \end{minipage}}%
  \endgroup\par\addvspace{\dimensioncardgap}%
}

\newcommand{\dimensionlabel}[2]{{%
  \setlength{\fboxsep}{1.5pt}%
  \colorbox{#1!6}{\textcolor{#1}{\textbf{\textit{#2}}}}%
}}

\newfloat{constructionalgorithm}{t}{loa}
\floatname{constructionalgorithm}{Algorithm}

\newcommand{\scorefirst}[1]{\cellcolor{orbiaRankFirst}\textbf{#1}}
\newcommand{\scoresecond}[1]{\cellcolor{orbiaRankSecond}\textbf{#1}}
\newcommand{\scorethird}[1]{\cellcolor{orbiaRankThird}\textbf{#1}}
\newcommand{\ranklegend}[2]{\textcolor{#1}{\raisebox{0.1ex}{\rule{0.75em}{0.65em}}}\nobreak\,\textbf{#2}}

\newcommand{\modellogo}[1]{\makebox[10pt][l]{\raisebox{-1.3pt}{\includegraphics[width=8pt,height=8pt,keepaspectratio]{assets/logo_#1}}}}

\pdfmapline{+Mulish-SemiBold-t1 Mulish-SemiBold "ECEncoding ReEncodeFont" <fonts/mulish/mulish-ec.enc <fonts/mulish/Mulish-SemiBold.ttf}
\DeclareFontFamily{T1}{orbiamulish}{}
\DeclareFontShape{T1}{orbiamulish}{m}{n}{<-> fonts/mulish/Mulish-SemiBold-t1}{}
\newcommand{\findingfont}{\fontencoding{T1}\fontfamily{orbiamulish}\fontseries{m}\fontshape{n}\selectfont}

\newcommand{\byes}{\textcolor{reportAccent}{$\checkmark$}}
\newcommand{\bno}{\textcolor{muted}{$\times$}}
\newcommand{\btag}[2]{{\setlength{\fboxsep}{1pt}\colorbox{#1!12}{\textcolor{#1}{\strut{\referencefont #2}}}}}
\newcommand{\bt}{\raisebox{-1.5pt}{\includegraphics[height=8pt]{assets/icon_text.png}}}
\newcommand{\ba}{\raisebox{-1.5pt}{\includegraphics[height=8pt,trim=60 60 60 60,clip]{assets/icon_action.png}}}
\newcommand{\bc}{\raisebox{-1.5pt}{\includegraphics[height=8pt,trim=40 70 40 70,clip]{assets/icon_camera.png}}}
\definecolor{datareal}{HTML}{3478C0}
\definecolor{dataself}{HTML}{26966F}
\definecolor{datasim}{HTML}{9362BE}
\definecolor{datagen}{HTML}{D28A28}
\newcommand{\bdata}[2]{{\setlength{\fboxsep}{1.5pt}\colorbox{#1}{\textcolor{white}{\scriptsize\sffamily\bfseries\makebox[6pt]{\strut #2}}}}}
\newcommand{\breal}{\bdata{datareal}{R}}
\newcommand{\bself}{\bdata{dataself}{C}}
\newcommand{\bsim}{\bdata{datasim}{S}}
\newcommand{\bgen}{\bdata{datagen}{G}}
\newcommand{\brgb}{\btag{persistence}{RGB}}
\newcommand{\bdepth}{\btag{evidence}{Depth}}
\definecolor{refaction}{HTML}{BC5965}
\newcommand{\baction}{\btag{refaction}{Action}}
\newcommand{\bpose}{\btag{coherence}{Pose}}
\newcommand{\tablehead}[1]{{\bfseries\shortstack{#1}}}
\newcommand{\resulthead}[1]{{\fontsize{7.5}{9}\selectfont\bfseries\shortstack{#1}}}
\newcommand{\componenthead}[1]{{\fontsize{6}{7}\selectfont\bfseries\shortstack{#1}}}
\newenvironment{constructionsteps}{%
  \begin{itemize}
  \setlength{\itemsep}{3pt}
  \setlength{\parsep}{0pt}
  \renewcommand{\labelitemi}{\textbullet}%
}{\end{itemize}}
\definecolor{sourcevideo}{HTML}{9B6580}
\definecolor{sourcescannet}{HTML}{527EA6}
\definecolor{sourceue}{HTML}{B7854D}
\definecolor{sourceself}{HTML}{478D82}
\newcommand{\coloredstep}[2]{%
  \par\noindent
  \textcolor{#1}{\raisebox{0.12ex}{\rule{0.45em}{0.45em}}}%
  \hspace{0.45em}\textbf{\textit{#2}}\ \ignorespaces
}
\definecolor{metriccontrol}{HTML}{7664A7}
\definecolor{metricquality}{HTML}{AF657E}
\colorlet{metricgeometry}{coherence}
\colorlet{metricinput}{evidence}
\colorlet{metricrevisit}{persistence}
\definecolor{metriclong}{HTML}{647580}
\newcommand{\metriccard}[2]{%
  \par\noindent
  \tikz{\node[rounded corners=1pt,fill=#1!6,draw=none,
    inner xsep=6pt,inner ysep=4pt,
    text width=\dimexpr\linewidth-13pt\relax,align=left,
    text=#1!55!black,font=\findingfont\small] (metriclabel) {%
    #2};
    \draw[#1!65,line width=1.2pt] (metriclabel.north west)--(metriclabel.south west);}%
  \par\nobreak\noindent\ignorespaces
}
\newcounter{metriccardnumber}[subsection]
\newcommand{\numberedmetriccard}[2]{%
  \stepcounter{metriccardnumber}%
  \metriccard{#1}{\arabic{metriccardnumber}.\enspace#2}%
}
\colorlet{adaptercamera}{sourcescannet}
\colorlet{adapteraction}{sourceself}
\definecolor{adaptertext}{HTML}{AF7860}
\newcommand{\adaptermodel}[3]{%
  \par\noindent
  \raisebox{-1.3pt}{\includegraphics[width=10pt,height=10pt,keepaspectratio]{assets/logo_#2}}%
  \hspace{0.35em}\textcolor{#1!70!black}{\textbf{#3}}\ \ignorespaces
}

\newcommand{\tablelayout}[2]{\setlength{\tabcolsep}{#1}\renewcommand{\arraystretch}{#2}}
\newcommand{\protocoltableslayout}{%
  \par\addvspace{8pt}%
  \captionsetup{position=top,skip=4pt}%
}
\newenvironment{tablebody}[2]{\tablelayout{#1}{#2}\ignorespaces}{\ignorespacesafterend}
\newcommand{\middlecolumns}{\renewcommand{\tabularxcolumn}[1]{m{##1}}}
\tikzset{
  orbia prompt/.style={rounded corners=8pt,line width=0.8pt,inner xsep=11pt},
  orbia vlm prompt/.style={orbia prompt,draw=reportAccent!45!gray,fill=reportAccent!3,inner ysep=7pt},
  orbia t2v prompt/.style={orbia prompt,draw=reportAccent!45!gray,fill=reportAccent!4,inner ysep=9pt}
}
\newenvironment{promptbody}{%
  \renewcommand{\ttdefault}{cmtt}%
  \renewcommand{\textbf}[1]{{\rmfamily\bfseries ##1}}%
  \ignorespaces
}{\ignorespacesafterend}
\newcommand{\tightfigurecaption}{\setlength{\abovecaptionskip}{4pt}}
\newcommand{\tightpromptcaption}{\tightfigurecaption\setlength{\belowcaptionskip}{0pt}}
\newcommand{\algorithmspacing}{\setlength{\itemsep}{2pt}\setlength{\parsep}{0pt}\setlength{\topsep}{3pt}}
\newenvironment{evaluationparagraphs}{\setlength{\parskip}{7pt}\ignorespaces}{\par\ignorespacesafterend}
\newenvironment{dimensioncards}{\setlength{\parskip}{0pt}\ignorespaces}{\ignorespacesafterend}
\makeatletter
\newenvironment{extendedresults}{%
  \raggedbottom\setlength{\@fptop}{0pt}\setlength{\@fpsep}{14pt}%
  \setcounter{topnumber}{5}\setcounter{totalnumber}{6}%
  \ignorespaces
}{\par\ignorespacesafterend}
\makeatother

\makeatletter
\g@addto@macro\UrlBreaks{\do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j\do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w\do\x\do\y\do\z\do\A\do\B\do\C\do\D\do\E\do\F\do\G\do\H\do\I\do\J\do\K\do\L\do\M\do\N\do\O\do\P\do\Q\do\R\do\S\do\T\do\U\do\V\do\W\do\X\do\Y\do\Z\do\0\do\1\do\2\do\3\do\4\do\5\do\6\do\7\do\8\do\9}
\makeatother
\setlength{\emergencystretch}{2em}
\renewcommand{\topfraction}{0.95}
\renewcommand{\textfraction}{0.05}
\setcounter{topnumber}{3}
\setcounter{totalnumber}{5}

\makeatletter
\newcommand{\orbiatitlepage}{%
  \addtocontents{toc}{\protect\setcounter{tocdepth}{-1}}%
  \maketitle
  \vspace{0.3cm}
  \input{figures/teaser}%
  \clearpage
  \reportabstract
  \vspace{0.2cm}
}
\newcommand{\orbiaappendix}{%
  \clearpage
  \appendix
  \addtocontents{toc}{\protect\setcounter{tocdepth}{3}}%
  \section*{Appendix}%
  \begingroup
  \color{orbiareview}%
  \hypersetup{linkcolor=orbiareview}%
  \fontsize{10}{14}\selectfont
  \renewcommand{\l@subsection}{\@dottedtocline{2}{1.5em}{2.9em}}%
  \renewcommand{\l@subsubsection}{\@dottedtocline{3}{4.4em}{3.6em}}%
  \@starttoc{toc}%
  \endgroup
  \clearpage
}
\newcommand{\orbiareferences}[1]{%
  \clearpage
  \begingroup
  \small
  \bibliographystyle{orbia-plainnat}%
  \bibliography{#1}%
  \endgroup
}
\makeatother
\endinput

